Rethinking Value Function Learning for Generalization in Reinforcement Learning

Our work focuses on training RL agents on multiple visually diverse environments to improve observational generalization performance. In prior methods, policy and value networks are separately optimized using a disjoint network architecture to avoid interference and obtain a more accurate value function. We identify that a value network in the multi-environment setting is more challenging to optimize and prone to memorizing the training data than in the conventional single-environment setting. In addition, we find that appropriate regularization on the value network is necessary to improve both training and test performance. To this end, we propose Delayed-Critic Policy Gradient (DCPG), a policy gradient algorithm that implicitly penalizes value estimates by optimizing the value network less frequently with more training data than the policy network. This can be implemented using a single unified network architecture. Furthermore, we introduce a simple self-supervised task that learns the forward and inverse dynamics of environments using a single discriminator, which can be jointly optimized with the value network. Our proposed algorithms significantly improve observational generalization performance and sample efficiency on the Procgen Benchmark.

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/algorithms/dcpg.tex <==
\begin{algorithm}[h]
	\small
	\caption{\cyan{Dynamics-aware} Delayed-Critic Policy Gradient (\cyan{D}DCPG)}
	\begin{algorithmic}[1]
	\Require Policy network $\pi_\theta$, value network $V_\theta$, \cyan{dynamics discriminator $f_\theta$}
    	\For{phase = $1, 2, \ldots $}
    	\State Initialize buffer $\mathcal{B}$
    	\For{iter = $1, 2, \ldots, N_\pi$} \Comment{Policy phase}
    	\State Sample trajectories $\tau$ using $\pi_\theta$ and compute value function target $\hat{R}_t$ for each state $s_t \in \tau$
    	\For{epoch = $1, 2, \ldots, E_\pi$}
    	\State Optimize policy objective $J_\pi(\theta)$ and value regularizer $C_V(\theta)$ with $\tau$
    	\EndFor
	\State Add $(s_t, \cyan{a_t}, \hat{R}_t)$ to $\mathcal{B}$
    	\EndFor
	\For{iter = $1, 2, \ldots, E_\mathrm{aux}$} \Comment{Auxiliary phase}
	\State Optimize value objective $J_V(\theta)$, \cyan{dynamics objective $J_f(\theta)$}, and policy regularizer $C_\pi(\theta)$ with $\mathcal{B}$
	\EndFor
    	\EndFor
	\end{algorithmic}
	\label{alg:dcpg}
\end{algorithm}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/algorithms/dcpg_sep.tex <==
\begin{algorithm}[h]
	\small
	\caption{\cyan{Separate} Delayed-Critic Policy Gradient (\cyan{Separate} DCPG)}
	\begin{algorithmic}[1]
	\Require Policy network $\pi_\theta$, value network $V_\theta$, \cyan{separate value network $V_\phi$}
    	\For{phase = $1, 2, \ldots $}
    	\State Initialize buffer $\mathcal{B}$
    	\For{iter = $1, 2, \ldots, N_\pi$} \Comment{Policy phase}
    	\State Sample trajectories $\tau$ using $\pi_\theta$
	\State Compute value function targets $\hat{R}_{t, \theta}$ \cyan{and $\hat{R}_{t, \phi}$} for each state $s_t \in \tau$
    	\For{epoch = $1, 2, \ldots, E_\pi$}
    	\State Optimize policy objective $J_\pi(\theta)$ and value regularizer $C_V(\theta)$ with $\tau$
	\State \cyan{Optimize value objective $J_V(\phi)$ with $\tau$}
    	\EndFor
	\State Add $(s_t, \hat{R}_{t, \theta}, \cyan{\hat{R}_{t, \phi}})$ to $\mathcal{B}$
    	\EndFor
	\For{iter = $1, 2, \ldots, E_\mathrm{aux}$} \Comment{Auxiliary phase}
	\State Optimize value objective $J_V(\theta)$ and policy regularizer $C_\pi(\theta)$ with $\mathcal{B}$
	\State \cyan{Optimize value objective $J_V(\phi)$ with $\mathcal{B}$}
	\EndFor
    	\EndFor
	\end{algorithmic}
	\label{alg:dcpg_sep}
\end{algorithm}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/algorithms/ppg.tex <==
\begin{algorithm}[h]
	\small
	\caption{Phasic Policy Gradient (PPG)}
	\begin{algorithmic}[1]
	\Require Policy network $\pi_\theta$, value network $V_\phi$, auxiliary value head $V_\theta$
    	\For{phase = $1, 2, \ldots $}
    	\State Initialize buffer $\mathcal{B}$
    	\For{iter = $1, 2, \ldots, N_\pi$} \Comment{Policy phase}
    	\State Sample trajectories $\tau$ using $\pi_\theta$ and compute value function target $\hat{R}_t$ for each state $s_t \in \tau$
    	\For{epoch = $1, 2, \ldots, E_\pi$}
    	\State Optimize policy objective $J_\pi(\theta)$ and value objective $J_V(\phi)$ with $\tau$
    	\EndFor
	\State Add $(s_t, \hat{R}_t)$ to $\mathcal{B}$
    	\EndFor
	\For{iter = $1, 2, \ldots, E_\mathrm{aux}$} \Comment{Auxiliary phase}
	\State Optimize value objective $J_V(\phi)$, auxiliary objective $J_\mathrm{aux}(\theta)$, and policy regularizer $C_\pi(\theta)$ with $\mathcal{B}$
	\EndFor
    	\EndFor
	\end{algorithmic}
	\label{alg:ppg}
\end{algorithm}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/dcpg_hp.tex <==
\begin{table}[h]
    \centering
    \caption{DCPG-specific hyperparameter.}
    \begin{tabular}{lc}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Value regularizer coefficient ($\beta_V$)& 1.0 \\
    \bottomrule
    \end{tabular}
    \label{tab:dcpg_hp}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/ppg_hp1.tex <==
\begin{table}[h]
    \centering
    \caption{PPO hyperparameters for PPG.}
    \begin{tabular}{lc}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Discount factor ($\gamma$) & 0.999 \\
    GAE smoothing parameter ($\lambda$) & 0.95 \\
    \# timesteps per rollout & 256 \\
    \# minibatches per epoch & 8 \\
    Entropy bonus & 0.01 \\
    PPO clip range ($\epsilon$) & 0.2 \\
    Reward normalization? & Yes \\
    Learning rate & 5e-4 \\
    \# workers & 1 \\
    \# environments per worker & 64 \\
    Total timesteps & 25M \\
    LSTM? & No \\
    Frame stack? & No \\
    \bottomrule
    \end{tabular}
    \label{tab:ppg_hp1}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/ppg_hp2.tex <==
\begin{table}[h]
    \centering
    \caption{PPG-specific hyperparameters.}
    \begin{tabular}{lc}
    \toprule
    Hyperparameter & Value \\
    \midrule
    \# policy phases per auxiliary phase ($N_\pi$) & 32 \\
    \# policy epochs ($E_\pi$) & 1 \\
    \# value epochs ($E_V$) & 1 \\
    \# auxiliary epochs ($E_\mathrm{aux}$) & 6 \\
    Policy regularizer coefficient ($\beta_\pi$)& 1.0 \\
    \# minibatches per auxiliary epoch per $N_\pi$ & 16 \\
    \bottomrule
    \end{tabular}
    \label{tab:ppg_hp2}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/ppo_hp.tex <==
\begin{table}[h]
    \centering
    \caption{PPO hyperparameters.}
    \label{tab:ppo_hp}
    \begin{tabular}{lc}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Discount factor ($\gamma$) & 0.999 \\
    GAE smoothing parameter ($\lambda$) & 0.95 \\
    \# timesteps per rollout & 256 \\
    \# epochs per rollout & 3 \\
    \# minibatches per epoch & 8 \\
    Entropy bonus & 0.01 \\
    PPO clip range ($\epsilon$) & 0.2 \\
    Reward normalization? & Yes \\
    Learning rate & 5e-4 \\
    \# workers & 1 \\
    \# environments per worker & 64 \\
    Total timesteps & 25M \\
    LSTM? & No \\
    Frame stack? & No \\
    \bottomrule
    \end{tabular}
    \label{tab:ppo_hp}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_daac.tex <==
\begin{table}[H]
	\centering
	\caption{PPO-normalized train and test scores of DAAC and IDAAC. Each agent is trained on 200 training levels for 25M environment steps. The mean and standard deviation are computed over 10 different runs.}
    	\begin{tabular}{l|rr}
	\toprule
	 & DAAC & IDAAC \\
	\midrule
	PPO-norm train score (\%) & 104.4 $\pm$ 4.1 & 99.7 $\pm$ 5.4 \\
	PPO-norm test score (\%) & 136.7 $\pm$ 7.6 & 129.9 $\pm$ 7.8 \\
	\bottomrule
	\end{tabular}
    	\label{tab:procgen_daac}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_dcpg_sep.tex <==
\begin{table}[H]
	\centering
	\caption{PPO-normalized training and test scores of PPG, Separate DCPG, and DCPG on all 16 Procgen games. Each agent is trained on 200 training levels for 25M environment steps. The mean and standard deviation are computed over 10 different runs.}
    	\begin{tabular}{l|>{\raggedleft}p{2cm}>{\raggedleft}p{2.4cm}>{\raggedleft}p{2cm}}
	\toprule
	 & PPG & Separate DCPG & DCPG \\
	\midrule
	PPO-norm train score (\%) & 136.7 $\pm$ 4.4 & 147.5 $\pm$ 1.9 & \textbf{152.7} $\pm$ \textbf{4.4} \\
	PPO-norm test score (\%) & 160.3 $\pm$ 6.3 & 174.4 $\pm$ 4.9 & \textbf{184.5} $\pm$ \textbf{5.2} \\
	\bottomrule
	\end{tabular}
    	\label{tab:procgen_dcpg_sep}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_regularization.tex <==
\begin{table}[h]
	\centering
	\caption{PPO-normalized training and test scores of PPG, PPG+DR, and PPG+AR. Each agent is trained on 200 training levels for 25M environment steps. The mean and standard deviation are computed over 10 different runs.}
    	\begin{tabular}{l|rrr}
	\toprule
	 & PPG & PPG+DR & PPG+AR  \\
	\midrule
	PPO-norm train score (\%) & 136.7 $\pm$ 4.4 & 146.8 $\pm$ 1.4 & 146.7 $\pm$ 2.6 \\
	PPO-norm test score (\%) & 160.3 $\pm$ 6.3 & 168.0 $\pm$ 5.8 & 169.9 $\pm$ 6.9 \\
	\bottomrule
	\end{tabular}
	\label{tab:procgen_regularization}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_ssl_count.tex <==
\begin{table}[h]
	\centering
	\caption{The number of OOD actions classified as valid for DCPG+F, DCPG+FI, and DDCPG on BigFish. Each agent is trained on 200 training levels for 25M environment steps.}
    	\begin{tabular}{l|rrr}
	\toprule
	 & DCPG+F & DCPG+FI & DDCPG \\
	\midrule
	\# OOD actions ($\downarrow$) & 7.05 $\pm$ 1.47 & 2.49 $\pm$ 1.38 & \textbf{0.74} $\pm$ \textbf{0.75} \\
	\bottomrule
	\end{tabular}
    	\label{tab:procgen_ssl_count}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_ssl_full.tex <==
\begin{table}[h]
	\centering
	\caption{PPO-normalized training and test scores of DCPG and DCPG with dynamics learning on all 16 Procgen games. Each agent is trained on 200 training levels for 25M environment steps. The mean and standard deviation are computed over 10 different runs.}
    	\adjustbox{max width=\textwidth}{
	\begin{tabular}{l|rrrrr}
	\toprule
	 & DCPG & DCPG+F & DCPG+I & DCPG+FI & DDCPG \\
	\midrule
	PPO-norm train score (\%) & 148.9 $\pm$ 4.3 & 150.6 $\pm$ 3.1 & 149.1 $\pm$ 3.4 & 150.5 $\pm$ 2.5 & \textbf{152.7} $\pm$ \textbf{4.4} \\
	PPO-norm test score (\%) & 184.5 $\pm$ 5.2 & 195.9 $\pm$ 7.7 & 185.5 $\pm$ 6.5 & 194.6 $\pm$ 6.2 & \textbf{202.2} $\pm$ \textbf{10.2} \\
	\bottomrule
	\end{tabular}}
    	\label{tab:procgen_ssl_full}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_ssl_ppg.tex <==
\begin{table}[h]
	\centering
	\caption{PPO-normalized test scores of PPG, DPPG, DCPG, and DDCPG on all 16 Procgen games. Each agent is trained on 200 training levels for 25M environment steps. The mean and standard deviation are computed over 10 different runs.}
    	\begin{tabular}{l|rrrr}
	\toprule
	 & PPG & DPPG & DCPG & DDCPG \\
	\midrule
	PPO-norm score (\%) & 160.3 $\pm$ 6.3 & 171.7 $\pm$ 4.9 & 184.5 $\pm$ 5.2 & 202.2 $\pm$ 10.2  \\
	\bottomrule
	\end{tabular}
    	\label{tab:procgen_ssl_ppg}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_test.tex <==
\begin{table}[t]
    \centering
    \caption{Average test returns of each method on all 16 Procgen games. Each agent is trained on 200 training levels for 25M environment steps and evaluated on 100 unseen test levels. The mean and standard deviation are computed over 10 different runs.}
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{l|rrrrr|rr}
        \toprule
        Environment & PPO & UCB-DrAC & PLR & DAAC\tablefootnote{Results reported in the original paper use a different hyperparameter setting for each game.} & PPG & DCPG & DDCPG \\
        \midrule
        BigFish & 3.4 $\pm$ 1.0 & 6.6 $\pm$ 2.5 & 10.8 $\pm$ 2.5 & 15.3 $\pm$ 3.0 & 16.4 $\pm$ 2.0 & 23.1 $\pm$ 2.3 & 25.9 $\pm$ 2.3 \\
        BossFight & 7.4 $\pm$ 0.7 & 7.2 $\pm$ 1.0 & 8.8 $\pm$ 0.7 & 9.5 $\pm$ 0.8 & 10.4 $\pm$ 0.6 & 10.2 $\pm$ 0.4 & 10.6 $\pm$ 0.5 \\
        CaveFlyer & 5.2 $\pm$ 0.6 & 4.4 $\pm$ 0.8 & 6.3 $\pm$ 0.7 & 5.1 $\pm$ 0.6 & 7.7 $\pm$ 0.7 & 6.3 $\pm$ 0.4 & 6.0 $\pm$ 0.3 \\
        Chaser & 5.5 $\pm$ 0.8 & 6.7 $\pm$ 0.5 & 7.5 $\pm$ 0.8 & 6.3 $\pm$ 0.8 & 8.9 $\pm$ 0.9 & 9.7 $\pm$ 0.4 & 9.9 $\pm$ 0.6 \\
        Climber & 5.5 $\pm$ 0.6 & 6.2 $\pm$ 0.6 & 6.4 $\pm$ 0.5 & 7.4 $\pm$ 0.5 & 8.1 $\pm$ 0.4 & 8.5 $\pm$ 0.7 & 9.3 $\pm$ 0.7  \\
        CoinRun & 8.8 $\pm$ 0.3 & 8.6 $\pm$ 0.4 & 8.9 $\pm$ 0.3 & 9.3 $\pm$ 0.2 & 8.9 $\pm$ 0.3 & 8.5 $\pm$ 0.4 & 8.4 $\pm$ 0.3 \\
        Dodgeball & 1.9 $\pm$ 0.3 & 4.5 $\pm$ 1.4 & 2.2 $\pm$ 0.4 & 3.2 $\pm$ 0.5 & 3.6 $\pm$ 0.7 & 6.7 $\pm$ 0.4 & 9.0 $\pm$ 1.6 \\
        FruitBot & 27.5 $\pm$ 1.5 & 26.9 $\pm$ 1.7 & 27.7 $\pm$ 1.3 & 28.5 $\pm$ 1.4 & 29.1 $\pm$ 1.0 & 29.0 $\pm$ 1.2 & 28.8 $\pm$ 0.6 \\
        Heist & 2.6 $\pm$ 0.6 & 3.4 $\pm$ 1.0 & 3.1 $\pm$ 0.6 & 3.0 $\pm$ 0.5 & 2.8 $\pm$ 0.5 & 3.3 $\pm$ 0.5 & 4.4 $\pm$ 0.8 \\
        Jumper & 5.7 $\pm$ 0.4 & 5.6 $\pm$ 0.4 & 5.9 $\pm$ 0.4 & 5.8 $\pm$ 0.4 & 6.0 $\pm$ 0.4 & 6.2 $\pm$ 0.5 & 6.4 $\pm$ 0.4 \\
        Leaper & 5.6 $\pm$ 1.5 & 3.6 $\pm$ 0.7 & 7.3 $\pm$ 0.2 & 8.2 $\pm$ 1.1 & 7.2 $\pm$ 2.4 & 6.9 $\pm$ 1.7 & 6.8 $\pm$ 1.5 \\
        Maze & 5.3 $\pm$ 0.7 & 5.7 $\pm$ 1.1 & 5.6 $\pm$ 0.5 & 5.6 $\pm$ 0.6 & 5.3 $\pm$ 0.4 & 5.7 $\pm$ 0.7 & 6.5 $\pm$ 0.6 \\
        Miner & 9.2 $\pm$ 0.6 & 10.1 $\pm$ 0.7 & 9.4 $\pm$ 0.7 & 4.4 $\pm$ 1.1 & 7.6 $\pm$ 0.7 & 9.1 $\pm$ 0.8 & 10.6 $\pm$ 0.5 \\
        Ninja & 5.7 $\pm$ 0.5 & 5.7 $\pm$ 0.5 & 7.1 $\pm$ 0.5 & 6.7 $\pm$ 0.7 & 6.7 $\pm$ 0.4 & 6.3 $\pm$ 0.6 & 6.6 $\pm$ 0.5 \\
        Plunder & 5.0 $\pm$ 0.5 & 8.1 $\pm$ 1.5 & 8.7 $\pm$ 1.3 & 5.6 $\pm$ 0.6 & 13.7 $\pm$ 1.7 & 13.7 $\pm$ 1.3 & 12.9 $\pm$ 2.5 \\
        StarPilot & 25.8 $\pm$ 2.0 & 27.0 $\pm$ 3.2 & 24.9 $\pm$ 3.6 & 35.9 $\pm$ 3.3 & 44.8 $\pm$ 2.6 & 46.1 $\pm$ 2.1 & 46.6 $\pm$ 4.1 \\
        \midrule
        PPO-norm score (\%) & 100.0 $\pm$ 3.1 & 120.7 $\pm$ 10.7 & 130.0 $\pm$ 6.0 & 136.7 $\pm$ 7.6 & 160.3 $\pm$ 6.3 & \textbf{184.5} $\pm$ \textbf{5.2} & \textbf{202.2} $\pm$ \textbf{10.2} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:procgen_test}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_test_ssl.tex <==
\begin{table}[h]
	\small
	\centering
	\caption{PPO-normalized score of each method with dynamics learning on all 16 Procgen games. Each agent is trained on 200 training levels for 25M environment steps and evaluated on 100 unseen test levels. The mean and standard deviation are computed over 10 different runs.}
    	\begin{tabular}{l|rrrrr}
	\toprule
	 & DCPG & DCPG+F & DCPG+I & DCPG+FI & DDCPG \\
	\midrule
	PPO-norm score (\%) & 184.5 $\pm$ 5.2 & 195.9 $\pm$ 7.7 & 185.5 $\pm$ 6.5 & 194.6 $\pm$ 6.2 & \textbf{202.2} $\pm$ \textbf{10.2} \\
	\bottomrule
	\end{tabular}
    	\label{tab:procgen_test_ssl}
\end{table}

==> Rethinking Value Function Learning for Generalization in Reinforcement Learning/tables/procgen_train.tex <==
\begin{table}[H]
    \centering
    \caption{Average training returns of each method on all 16 Procgen games. Each agent is trained on 200 training levels for 25M environment steps and evaluated on the same training levels. The mean and standard deviation are computed over 10 different runs.}
    \label{tab:procgen_train}
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{l|rrrrr|rr}
        \toprule
        Environment & PPO & UCB-DrAC & PLR & DAAC & PPG & DCPG & DDCPG \\
        \midrule
        BigFish & 11.0 $\pm$ 1.7 & 12.2 $\pm$ 3.1 & 13.6 $\pm$ 3.0 & 18.4 $\pm$ 3.3 & 24.1 $\pm$ 1.6 & {32.8} $\pm$ {2.0} & {31.8} $\pm$ {2.1} \\
        BossFight & 7.9 $\pm$ 0.7 & 8.2 $\pm$ 0.7 & 8.8 $\pm$ 0.7 & 9.9 $\pm$ 0.7 & {11.1} $\pm$ {0.3} & 10.7 $\pm$ 0.6 & 11.0 $\pm$ 0.5 \\
        CaveFlyer & 7.1 $\pm$ 0.9 & 6.0 $\pm$ 0.9 & 7.3 $\pm$ 0.5 & 6.8 $\pm$ 0.8 & {10.0} $\pm$ {0.5} & 9.0 $\pm$ 0.5 & 9.0 $\pm$ 0.3 \\
        Chaser & 6.4 $\pm$ 0.8 & 7.3 $\pm$ 0.7 & 8.0 $\pm$ 0.6 & 6.4 $\pm$ 1.0 & 10.0 $\pm$ 0.7 & {10.4} $\pm$ {0.6} & {10.6} $\pm$ {0.5} \\
        Climber & 8.4 $\pm$ 0.5 & 8.4 $\pm$ 0.6 & 8.6 $\pm$ 0.6 & 9.3 $\pm$ 0.6 & 10.9 $\pm$ 0.4 & {11.3} $\pm$ {0.5} & {11.9} $\pm$ {0.4}  \\
        CoinRun & 9.6 $\pm$ 0.1 & 9.5 $\pm$ 0.2 & 9.4 $\pm$ 0.3 & 9.9 $\pm$ 0.1 & {10.0} $\pm$ {0.1} & 9.9 $\pm$ 0.1 & 9.9 $\pm$ 0.1 \\
        Dodgeball & 5.5 $\pm$ 0.7 & 8.0 $\pm$ 1.2 & 5.1 $\pm$ 0.8 & 6.4 $\pm$ 0.9 & 7.9 $\pm$ 0.7 & {11.9} $\pm$ {1.4} & {14.1} $\pm$ {1.1} \\
        FruitBot & 29.9 $\pm$ 0.5 & 29.1 $\pm$ 1.3 & 28.3 $\pm$ 1.3 & 29.8 $\pm$ 1.1 & {31.9} $\pm$ 0.4 & {31.9} $\pm$ 0.4 & 31.1 $\pm$ 0.8 \\
        Heist & 7.6 $\pm$ 0.6 & 7.2 $\pm$ 0.6 & 8.0 $\pm$ 0.5 & 4.9 $\pm$ 0.8 & 7.4 $\pm$ 0.6 & {8.6} $\pm$ {0.4} & {9.4} $\pm$ {0.4}\\
        Jumper & 8.7 $\pm$ 0.3 & 8.4 $\pm$ 0.5 & 8.6 $\pm$ 0.3 & 8.8 $\pm$ 0.3 & {9.1} $\pm$ {0.3} & 8.6 $\pm$ 0.4 & 8.9 $\pm$ 0.3 \\
        Leaper & 5.8 $\pm$ 1.5 & 3.6 $\pm$ 1.1 & 7.0 $\pm$ 0.6 & {8.8} $\pm$ {1.0} & 8.2 $\pm$ 2.9 & 8.4 $\pm$ 2.3 & 8.4 $\pm$ 2.3 \\
        Maze & 9.3 $\pm$ 0.3 & 8.5 $\pm$ 0.5 & 9.2 $\pm$ 0.4 & 5.7 $\pm$ 0.4 & 9.5 $\pm$ 0.3 & {9.6} $\pm$ {0.2} & {9.7} $\pm$ {0.2}\\
        Miner & 12.8 $\pm$ 0.2 & 12.4 $\pm$ 0.3 & 11.4 $\pm$ 0.6 & 4.7 $\pm$ 0.7 & 11.6 $\pm$ 0.4 & 12.7 $\pm$ 0.1 & {12.8} $\pm$ {0.1} \\
        Ninja & 7.8 $\pm$ 0.4 & 7.5 $\pm$ 1.0 & 8.2 $\pm$ 0.4 & 9.0 $\pm$ 0.2 & {9.8} $\pm$ {0.2} & 9.6 $\pm$ 0.1 & 9.6 $\pm$ 0.2 \\
        Plunder & 6.2 $\pm$ 0.7 & 9.2 $\pm$ 1.3 & 11.0 $\pm$ 1.1 & 5.9 $\pm$ 0.6 & 14.5 $\pm$ 2.1 & {15.7} $\pm$ {1.8} & {16.0} $\pm$ {2.3} \\
        StarPilot & 29.9 $\pm$ 3.6 & 30.2 $\pm$ 2.4 & 26.3 $\pm$ 3.2 & 39.0 $\pm$ 2.5 & 48.4 $\pm$ 3.4 & {50.5} $\pm$ {1.8} & {50.8} $\pm$ {4.0} \\
        \midrule
       PPO-norm score (\%) & 100.0 $\pm$ 2.5 & 102.6 $\pm$ 3.4 & 107.9 $\pm$ 3.5 & 104.4 $\pm$ 4.1 & 136.7 $\pm$ 4.4 & \textbf{148.9} $\pm$ \textbf{4.3} & \textbf{152.7} $\pm$ \textbf{4.4} \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/dcpg_hp.tex <==
\begin{table}[h]
    \centering
    \caption{DCPG-specific hyperparameter.}
    \begin{tabular}{lc}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Value regularizer coefficient ($\beta_V$)& 1.0 \\
    \bottomrule
    \end{tabular}
    \label{tab:dcpg_hp}
\end{table}

==> tables/ppg_hp1.tex <==
\begin{table}[h]
    \centering
    \caption{PPO hyperparameters for PPG.}
    \begin{tabular}{lc}
    \toprule
    Hyperparameter & Value \\
    \midrule
    Discount factor ($\gamma$) & 0.999 \\
    GAE smoothing parameter ($\lambda$) & 0.95 \\
    \# timesteps per rollout & 256 \\
    \# minibatches per epoch & 8 \\
    Entropy bonus & 0.01 \\
    PPO clip range ($\epsilon$) & 0.2 \\
    Reward normalization? & Yes \\
    Learning rate & 5e-4 \\
    \# workers & 1 \\
    \# environments per worker & 64 \\
    Total timesteps & 25M \\
    LSTM? & No \\
    Frame stack? & No \\
    \bottomrule
    \end{tabular}
    \label{tab:ppg_hp1}
\end{table}
